RL Tango: Reinforcing Generator and Verifier Together for Language Reasoning

Reinforcement learning (RL) has recently emerged as a compelling approach for enhancing the reasoning capabilities of large language models (LLMs), where an LLM generator serves as a policy guided by a verifier (reward model). However, current RL post-training methods for LLMs typically use verifiers that are fixed (rule-based or frozen pretrained) or trained discriminatively via supervised fine-tuning (SFT). Such designs are susceptible to reward hacking and generalize poorly beyond their training distributions. To overcome these limitations, we propose Tango, a novel framework that uses RL to concurrently train both an LLM generator and a verifier in an interleaved manner. A central innovation of Tango is its generative, process-level LLM verifier, which is trained via RL and co-evolves with the generator. Importantly, the verifier is trained solely based on outcome-level verification correctness rewards without requiring explicit process-level annotations. This generative RL-trained verifier exhibits improved robustness and superior generalization compared to deterministic or SFT-trained verifiers, fostering effective mutual reinforcement with the generator. Extensive experiments demonstrate that both components of Tango achieve state-of-the-art results among 7B/8B-scale models: the generator attains best-in-class performance across five competition-level math benchmarks and four challenging out-of-domain reasoning tasks, while the verifier leads on the ProcessBench dataset. Remarkably, both components exhibit particularly substantial improvements on the most difficult mathematical reasoning problems. Code is at: https://github.com/kaiwenzha/rl-tango.

==> tabs/license.tex <==
\vspace{-2mm}
\begin{table}[!ht]
% \setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.1}
\caption{\textbf{Licenses for external assets} used in our experiments.}
\label{tab:license_assets}
\small
\begin{center}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{lll}
\toprule[1pt]
\textbf{Asset} & \textbf{Type} & \textbf{License / Terms} \\
\midrule
Qwen2.5-Math-7B~\cite{yang2024qwen25mathtechnicalreportmathematical} & Model & Apache 2.0 \\
Qwen2.5-7B~\cite{yang2024qwen25} & Model & Apache 2.0 \\
Llama-3.1-70B-Instruct~\cite{grattafiori2024llama} & Model & Llama 3.1 Community License \\
Qwen2.5-1.5B~\cite{yang2024qwen25} & Model & Apache 2.0 \\
Eurus-2-SFT-Data~\cite{cui2025process} & Dataset & MIT \\
Eurus-2-RL-Data~\cite{cui2025process} & Dataset & MIT \\
MATH 500~\cite{lightman2023let} & Dataset & MIT \\
AIME 2024~\cite{aime2024} & Dataset & Apache 2.0 \\
AIME 2025~\cite{aime2025} & Dataset & MIT \\
AMC 2023~\cite{amc2023} & Dataset & Apache 2.0 \\
OlympiadBench~\cite{he2024olympiadbench} & Dataset & Apache 2.0 \\
BoardgameQA~\cite{kazemi2023boardgameqa} & Dataset & CC-BY 4.0 \\
CRUXEval~\cite{gu2024cruxeval} & Dataset & MIT \\
StrategyQA~\cite{geva2021did} & Dataset & MIT \\
TableBench~\cite{wu2025tablebench} & Dataset & Apache 2.0 \\
ProcessBench~\cite{zheng2024processbench} & Dataset & Apache 2.0 \\
veRL~\cite{sheng2024hybridflow_verl_codebase} & Codebase & Apache 2.0 \\
\bottomrule[1pt]
\end{tabular}}
\end{center}
\vspace{-4mm}
\end{table}

